Challenges and Opportunities for Global Cellular Connectivity

Traditional cellular service was designed for global connectivity, but business and logistical constraints led to its fragmentation, with deployments limited to individual countries and regions. Initiatives like Mobile Virtual Network Operators (MVNOs), Mobile Network Aggregators (MNAs), and regulations like ''roam-like-at-home'' have partially restored global service potential, though often at high costs in terms of user bills, application performance, and traffic efficiency. This paper makes two key contributions: first, it surveys the global cellular ecosystem, analyzing the strengths and weaknesses of major players using data from prior research, proprietary datasets, and public sources. Second, it argues that the technology for seamless global service exists in Local Breakout (LBO), a roaming architecture which allows user traffic to be routed directly to the Internet through the visited network, bypassing the home network and/or third-party infrastructures. However, LBO adoption is hindered by issues such as policy enforcement, billing, and Quality of Service (QoS) guarantees, rooted in a lack of trust between operators. The paper concludes by exploring technological advances that could enable LBO, and pave the way for truly global cellular connectivity.

==> sections/old_novel_research_questions.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Virtual (Global) Aggregators}
\label{sec:directions}
%%%%%%%%%%%%%%%%%%%%%%

%MV -- I think we can start more directly (also we need space - potential content for Intro)
%The seven different angles we capture in Table~\ref{tab:summary} back the perplexing reality that practically realizing global mobile connectivity with local breakout (i.e., towards a native-like service in the visited location) is (currently) an uphill struggle. 
%At the same time, the surge in global cellular IoT deployments and international travel returning to pre-pandemic levels translate into increasing end-user demand (and revenue potential) for seamless mobile connectivity experience globally, just as they might receive at home. 
%Several operator models have emerged to cater to this demand, all within the confines of the current cellular ecosystem trust model, and despite its (many) shortcoming that we identified in Table~\ref{tab:summary}.

%Fragmenting the operator's functionalities (control and data plane) and network realm (the core network, the \gls{ran}), and disconnecting from the (bygone) need of a single entity managing all these aspects and underlying infrastructure, most global operator models today overload the international roaming function to expand their footprint world-wide.

%In this section, we provide 
This section provides an overview of the \textbf{global} operational models we identified at the time of writing, and discuss 
%to which extent they tackle some of the aspects we brought forward as barriers (see Table~\ref{tab:summary}) towards achieving native-like connectivity globally, %in any visited location (\eg through local breakout roaming.  
%This exercise shows the potential to further advance these existing operational models by removing the barriers towards ultimately achieving a truly global operator model. 
Table~\ref{fig:mna_models} captures all the different operator models that we identified at the time of writing. \mvnote{update sentence once table is ready, aka validating each operating model with respect to the ideas from Table~\ref{tab:summary}. See an idea for a table I pasted from another paper}

\newcommand{\No}{\cellcolor{red!25}No\xspace}
\newcommand{\Yes}{\cellcolor{green!25}Yes\xspace}
\newcommand{\YesNo}{\cellcolor{orange!25}Yes*\xspace}
\newcommand{\NA}{\cellcolor[gray]{0.75}N/A\xspace}
\newcommand{\NoEmtpy}{\cellcolor{red!25}\xspace}
\newcommand{\YesEmtpy}{\cellcolor{green!25}\xspace}
\newcommand{\YesNoEmtpy}{\cellcolor{orange!25}\xspace}
\newcommand{\NAEmtpy}{\cellcolor[gray]{0.75}\xspace}
\begin{table}[t]
\footnotesize
\setlength\tabcolsep{3pt}
\caption{FIXME - just an idea of what we could have here.}
\label{tab:solutions}
\begin{tabular}{c | c c c c}
\toprule
    \multirow{4}{*}{\parbox{2.6cm}{\centering }}  
    & \multirow{4}{*}{\parbox{1.2cm}{\footnotesize \centering Trust}} 
    & \multirow{4}{*}{\parbox{1.0cm}{\footnotesize \centering Security}} 
    & \multirow{4}{*}{\parbox{1.0cm}{\footnotesize \centering Regulatory}} 
    & \multirow{4}{*}{\parbox{1.3cm}{\footnotesize \centering Billing}}  \\\\\\\\
\toprule
    Airalo & \No & \No & \No & \NA \\\hline
    1NCE & \Yes & \No & \No & \NA \\\hline    
    emnify & \Yes & \Yes & \No & \No \\\hline        
    Twilio & \Yes & \Yes & \No & \No \\\hline    
\bottomrule
\end{tabular}
% \vspace{-0.05in}
\end{table}


\begin{figure}[!t]
    \includegraphics[width=\columnwidth]{figures/global_models_mvno-mna.png}
    % \vspace{-6mm}
    \caption{\small Network operating models: MVNOs lacks ownership of radio spectrum resources; light/thick MVNOs rely on a single b-MNO, and the latter's roaming agreements for global service, while full MVNOs operate their own core network, and give global service through their own roaming agreements.
    MNAs run a limited part of the network (the \textit{light} -- only sales $<<$  the \textit{thick} -- limited core function $<<$ the \textit{full} -- all the core), and provide global service by exploiting the roaming agreements of several b-MNOs. }
    \label{fig:mna_models}
    \vspace{-0.2in}    
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{MNA Models}
\label{sec:mna_models}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mvnote{I think we need a new subsection title}
Pushing further the \gls{mvno} models, \glspl{mna} have emerged with the aim to deliver global connectivity to the end-user.
While ``traditional'' \glspl{mvno} have agreements with a single base \gls{mno} and typically operate only within one single economy, an \gls{mna} is an \gls{mvno} that exploits more than one base MNO -- usually across different economies -- and operates world-wide.   
In recent years, we have witnessed myriad flavors of \glspl{mna}, which exploit the coverage footprint of a handful of base operators. 
Some notable examples of \glspl{mna} include Google Fi, 1Global, Twilio/KORE, emnify or Airalo.
Under the MNA model, these operators reap the benefits of network softwarization and virtualization~\cite{jain22L25GC, luo21cellbricks, larrea23coreKube}, including eSIM technology or control/data-plane separation~\cite{alcala2022global}.
Operators such as Airalo and Holafly cater to international travelers in any visited location, and promise to deliver native-like quality of service, while operators such as emnify focus on globally connecting IoT vertical applications.  

These novel technologies enables a new era in global mobile connectivity, characterized by varying degrees of operational complexity, which we capture in Table~\ref{tab:summary}. 
Similarly to the case of \glspl{mvno}, we have seen (commercial) evidence of \glspl{mna} that rely on the core networks of base operators (\textit{Light \glspl{mna}}) or run their own (\textit{Full \glspl{mna}})~\cite{alcala2022global, yuan18mobicom} to provision their \gls{esim} profiles.
Both models gain access to (visited) radio access networks globally via interconnection through roaming hubs~\cite{lutu2020first}.
\textit{Thick MNAs} push this model further, and decouple the internet gateway location from both the base MNOs' and the visited operators' infrastructure. For example, Airalo~\cite{airalo} is a popular thick MNA~\cite{hyunseok2024unravelingairaloecosystem}, which has gained more than 5 million customers\footnote{https://www.airalo.com/about-us/about-airalo} since its inception in 2019. 
Emnify leverage a similar operational model focused on IoT-specific global connectivity: where they use seven different cloud locations as roaming breakout points, all from the same provider. 


\paragraph{Evolving from \gls{hr} roaming}
It is now general knowledge that global cellular service within the current ecosystem is enabled through the (international) roaming function, and that home-routed roaming is the preferred \gls{mno} configuration, even for 5G networks~\cite{fezeu2024roaming, mandalari2018experience, mandalari2022measuring}.
By extending the \gls{mvno} model towards aggregating base \glspl{mno} from different economies, some \glspl{mna} aim to reduce the performance penalty of \gls{hr} by dynamically changing the base MNO. 
This uses the same underlying trust model for international roaming within the cellular ecosystem. 
%Aggregating multiple base MNOs allows the \gls{mna}'s customers to dynamically change the base MNO to which they attach. 
This model of operation aggregates multiple \glspl{mno} from different countries to ultimately deliver service to end-users (almost?) anywhere in the world. 
The (dynamic) change of base MNOs depends on different factors, including policy, coverage or performance.

However, it is still unclear whether their performance is similar to that of native-like connectivity in a visited location (i.e., via a local provider in the visited location). 
Conversely, depending on the application they support, it is unclear if and how realizing native-like connectivity through local breakout might impact the \glspl{mna}'s respective end-users. 
We thus highlight here the limited knowledge within our community~\cite{hyunseok2024unravelingairaloecosystem, alcala2022global, xiao19mobisys, yuan18mobicom} around how these different models of MNAs cater to the need for global coverage for their end-users. 
We discuss next several of these aspects through the looking glass of the barriers in Table~\ref{tab:summary}.
\ael{I'd really like to attempt here a nice table where we can tie to the "challenges"/"barriers" we had in Table 1... but I also need to shringk considerably table 1, which feels a bit "bla" at this point, and could use more consolidation.}
In particular, we note that all these models build on top of the same unchanged trust model within the cellular ecosystem, where the home MNO is the sole "owner" of the end-user identity. 


\paragraph{Mapping the MNA Breakout Locations}
Previous work ran active measurements and mapped the breakout locations for specific client devices~\cite{mandalari2018experience, mandalari2022measuring, alcala2022global, vomhoff2024shortcut}.
The findings of these studies unveil how \glspl{mna} are gradually exploiting the idea of swapping base MNOs, depending on the end-user location, all in an effort to reduce the implications of the \gls{hr} roaming setup~\cite{mandalari2022measuring}.
Depending on their setup, \glspl{mna} achieve different levels of geo-spatial granularity in terms of the breakout locations.

\textbf{Continent-level breakout (e.g., Google Fi)}: 
Google Fi is a \textit{light MNA} that relies on T-Mobile in the US, and Three UK in Europe~\cite{alcala2022global}.
Fi targets users in the US, and also offers gloabal roaming coverage. 
For users traveling from the US to Spain, we find that Fi swapped the base MNO from T-Mobile to Three in the UK. 
The use of regional breakout in Europe on top of Three's network helps Fi to reduce significantly (i.e., by ) the delay their users experience in Europe.

\textbf{Country-level breakout (e.g., 1Global)}: 1Global (previously known as Truphone) is a \textit{full MNA}, operating their own core network, and aggregates separate individual MVNO agreements from the 9 nine economies where they register. 
1Global was, in fact, the closest -- to the best of our knowledge -- to deliver native-like mobile connectivity to global users~\cite{alcala2022global}. 
1Global achieve this by mapping the breakout point to the closest \gls{mvno} partnerships to the location where they aim to give service. 
Leveraging their mature setup with different MVNO partnerships in over 9 countries, 1Global was able to deliver the performance closest to the one provided by a local MNO in any of those countries. 

\textbf{Sponsored Roaming and Cloud Breakout (e.g., emnify, Twilio/KORE, Airalo):} 

\ael{@viktoria, could you please add some details on emnify based on already published material in \cite{vomhoffshortcut}/}

\ael{@daniel, could you please add some details about airalo based on the published material in arxiv? please also add the reference, many thanks!}

Airalo operates as a \textit{thick MNA}, leveraging the deployment of internet breakout gateways in third-party (cloud) network infrastructures that are decoupled from both the base and the visited MNOs. In theory, this mode of operation allows for the benefits of RBO, particularly the dynamic traffic routing and prioritization of gateways closer to the user. However, in practice, Airalo eSIMs are configured to statically route traffic through specific internet gateways, often resulting in geographically suboptimal data path. Airalo's performance measurement across 21 countries found that while RBO eSIMs offered better latency compared to HRR counterparts, they showed minimal improvement in bandwidth~\cite{jang2024unravelingairaloecosystem}. This highlights the challenge of RBO operations due to the need for a complex interplay of agreements among MNOs, IPX providers, and network infrastructure companies.



\ael{add here some more insights into the airalo paper, add the citation to the version in arxiv too}


\textbf{Research efforts (Cellbricks~\cite{luo21cellbricks}, PGPP\cite{schmitt2021pretty, schmitt2022decoupling}}
\ael{I think this should go to section 5, where we can discuss some ideas to tackle the shortcoming of the MNA models we analyzed... }



